Global Rewards in Restless Multi-Armed Bandits

Restless multi-armed bandits (RMAB) extend multi-armed bandits so pulling an arm impacts future states. Despite the success of RMABs, a key limiting assumption is the separability of rewards into a sum across arms. We address this deficiency by proposing restless-multi-armed bandit with global rewards (RMAB-G), a generalization of RMABs to global non-separable rewards. To solve RMAB-G, we develop the Linear- and Shapley-Whittle indices, which extend Whittle indices from RMABs to RMAB-Gs. We prove approximation bounds but also point out how these indices could fail when reward functions are highly non-linear. To overcome this, we propose two sets of adaptive policies: the first computes indices iteratively, and the second combines indices with Monte-Carlo Tree Search (MCTS). Empirically, we demonstrate that our proposed policies outperform baselines and index-based policies with synthetic data and real-world data from food rescue.

==> previous_writeup/algorithms.tex <==
\section{Matching with Restless Multi-Armed Bandits}
We describe complications arising in the matching scenario through a simple example that demonstrates the trade-off between what we call ``activity'' and the number of matches.  
We discuss how algorithms from vanilla RMABs can be applied to the matching scenario, and describe the application to a food rescue scenario. 

\subsection{Incorporating Matching}
We consider the RMAB framework applied to a matching context. 
In addition to local rewards, we consider a global reward function, $R_{G}: \mathcal{S}^N \times \mathcal{A}^N \rightarrow \mathbb{R}$, which pools together states and actions from different arms to produce an additional reward, and rename $R$ to $R_{\mathrm{i}}$ to allow for individual rewards for each arm. 
Our goal is to maximize the combined reward, balanced by some hyperparameter $\lambda$ which mediates the interaction between $R_{i}$, which we denote the \textit{activity}, and $R_{G}$, which we denote the \textit{matching} by learning a policy $\pi: \mathcal{S} \rightarrow \mathcal{A}$. 
Formally, we aim to maximize 
\begin{equation}
    \mathbb{E} _{(\mathbf{s},\mathbf{a})\sim (\mathcal{P},\pi)} \sum_{t=1}^{\infty} \gamma^{t} (R_{G}(\{s_{1}^{(t)} \cdots s_{N}^{(t)}\},\{a_{1}^{(t)} \cdots a_{N}^{(t)}\}) + \lambda  [\sum_{i=1}^{N} R_{i}(s_{i}^{(t)},a_{i}^{(t)})])
\end{equation}

We describe the global reward function, $G$, for matching in particular. 
At each time step, a request comes in, and the goal is to match this request with some arm. 
We consider the partition of $\mathcal{S}$ into two disjoint subsets: disinterested states, $D$, and engaged states $E$, $E \cup D = S, E \cap D = \varnothing$. 
Only arms with $s_{i}^{(t)} \in E$ and $a_{i}^{(t)}=1$ can be matched to the context. 
With a food rescue scenario, this corresponds to the idea that only volunteers who are both engaged and receive notification can be matched to a particular food rescue trip. 
Arm-request matching is stochastic, and we define the probability that an arm matches with a given request, given both $s_{i}^{(t)} \in E$ and $a_{i}^{(t)}=1$, as $p_{i}^{(t)} \in [0,1]$. 
Because of the difficulty in optimizing non-linear objective functions, we approximate the global matching objective function $G$, through the following: 
\begin{equation}
   R_{G}(\{s_{1}^{(t)} \cdots s_{N}^{(t)}\},\{a_{1}^{(t)} \cdots a_{N}^{(t)}\}) ~\simeq \sum_{i=1}^{N}  p_{i}^{(t)} a_{i}^{(t)} \mathbbm{1}[s_{i}^{(t)} \in E]
\end{equation}

In many matching scenarios, our goal is to maximize matches, while ensuring that some notion of active users or volunteers is maintained. 
To model this, we capture the notion of maximizing matches through our global reward function, $R_{G}$, while our reward function $R_{i}$ captures the level of engagement or activity for a user. 
Because the level of engagement is only a function of the state, rather than the actions, we let $R_{i}(s_{i}^{(t)},a_{i}^{(t)}) = R_{i}(s_{i}^{(t)})$. 
Using our previous definition for the global reward, we state our optimization problem, across all iterations $t$, as follows: 
\begin{equation}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle \mathbb{E} _{(\mathbf{s},\mathbf{a})\sim (\mathcal{P},\pi)} \sum\limits_{t=1}^{\infty} \gamma^{t} (\sum_{i=1}^{n} p_{i}^{(t)} a_{i}^{(t)} \mathbbm{1}[s_{i}^{(t)} \in E]  & + \lambda R_{i}(s_{i}^{(t)})) &\\
\text{subject to}&                                                & a_{i}^{(t)} \in [0,1]           &i=1 ,\dots, n\\
                 &                                                &
                 &t = 1 ,\dots,T\\
                 &\displaystyle\sum\limits_{i=1}^{N}              & a_{i}^{(t)} \leq K    &\forall t\\
\end{array}
\end{equation}
We note the flexibility of our approach; it captures various values of the probability of matching, $p_{i}^{(t)}$, and for any formulation of $R_{i}(s_{i}^{(t)})$. 
For example, state values can capture the benefit for arms being in various states; arms in detrimental states can have $R_{i}(s_{i}^{(t)})$ to be negative, such as volunteers being burned out in a food rescue scenario, while for beneficial states, such as engaged volunteers, $R_{i}(s_{i}^{(t)})$ can be positive. 
We also note that our formulation can capture time periods, $t$, where no matching requests arise. 
In such time intervals, we let $p_{i}^{(t)} = 0$, and we assume that whatever arms are pulled still incur a reward $R_{i}(s_{i}^{t})$. 

\subsection{Trade off between Activity and Matching}
We next note that maximizing the activity of arms, which we define as the arms being in a ``favorable'' state and corresponding to the reward $R_{i}$, is not necessarily aligned to maximize matching, which corresponds to the goal $G$. 
We present this through an example: 

\begin{example}
    Consider a simple $N=2$ arm system, with each arm being in one of two states, $0$ or $1$. 
    Suppose our reward is $R_{i}(0) = 0$ and $R_{i}(1)=1$, and let $D=\{0\}$ and $E=\{1\}$. 
    Therefore, both matching and activity benefit from keeping arms in the $1$ state. 
    Next, define the transition probabilities for the first arm as follows: 
    \begin{equation}
        P_{0}(a=0) =  [
        \begin{bmatrix}
        & \text{End State 0} & \text{End State 1} \\
          \text{Start State 0} & 1 & 0 \\
          \text{Start State 1} & 1 & 0 \\
        \end{bmatrix}
        ]
    \end{equation} 
    \begin{equation}
        P_{0}(a=1) = [
        \begin{bmatrix}
        & \text{End State 0} & \text{End State 1} \\
          \text{Start State 0} & 1-\epsilon & \epsilon \\
          \text{Start State 1} & 1-\epsilon & \epsilon \\
        \end{bmatrix}
        ]
    \end{equation}

    Additionally, let the transition probabilities for the second arm be as follows: 
    \begin{equation}
        P_{1}(a=0) =  [
        \begin{bmatrix}
        & \text{End State 0} & \text{End State 1} \\
          \text{Start State 0} & 1 & 0 \\
          \text{Start State 1} & 0 & 1 \\
        \end{bmatrix}
        ]
    \end{equation} 
    \begin{equation}
        P_{1}(a=1) = [
        \begin{bmatrix}
        & \text{End State 0} & \text{End State 1} \\
          \text{Start State 0} & 0 & 1 \\
          \text{Start State 1} & 0 & 1 \\
        \end{bmatrix}
        ]
    \end{equation}

    Suppose both arms start in state 0. Then the optimal strategy to maximize activity is to first pull arm 1, thereby guaranteeing $T-1$ reward for the remaining time periods, as this guarantees arm 1 will be in state 1. For every time period afterwards, we then pull arm 0, which will be in state 1 with probability $\epsilon$, giving us a total activity reward of $(T-1) + \epsilon T$. However, note that the global reward for matching is dependent on notifying active users. We only receive a reward for that in this situation if Agent 0 is active, which occurs $\epsilon T$ times, giving a total matching reward of $p \epsilon (T-2)$. 

    However, note that the optimal matching strategy is to repeatedly pull arm 1. This yields an activity of $T-1 \leq (T-1) \epsilon T$, but yields a matching reward of $p (T-1) \geq p \epsilon (T-2)$. 
    This demonstrates that the optimal activity and matching strategies are not necessarily aligned, and can potentially disagree on all but a constant number of actions. 
    
\end{example}

\subsection{Whittle Index Solution}
We note that we can optimize a combination of the matching and activity objective functions through the Whittle index algorithm~(Section \ref{sec:whittle}). 
In particular, we aim to solve 
\begin{equation}
    \sum_{i=1}^{N} p_{i}^{(t)} a_{i}^{(t)} \mathbbm{1}[s_{i}^{(t)} \in E] + \lambda R_{i}(s_{i}^{(t)})
\end{equation}
This can be viewed as a reward function, $R'(s_{i}^{(t)},a_{i}^{(t)}) = p_{i}^{(t)} a_{i}^{(t)} \mathbbm{1}[s_{i}^{(t)} \in E] + \lambda R_{i}(s_{i}^{(t)})$. 
Then our goal follows the standard Whittle index structure, where we aim to maximize 
\begin{equation}
   \sum_{t=1}^{\infty} \gamma{^t} (\sum_{i=1}^{N} R'(s_{i}^{(t)},a_{i}^{(t)}))
\end{equation}
We note that in our scenario, the combination of the two objective functions is linear in $a_{i}^{(t)}$, and so through prior work~\cite{glazebrook2006some}, such a formulation is indexable, allowing for us to use the Whittle index algorithm. 
Solving the Whittle index algorithm requires performing Q-iteration for each value of the subsidy, which requires $\mathcal{O}(|\mathcal{S}|^{2}|\mathcal{A}|)$, where $|\mathcal{S}|$ is the size of the state space, and $|A|$ is the size of the action space. 
If we assume it takes $M$ iterations to find the optimal subsidy, and that we need to find the subsidy for each state-agent combination, then it takes $\mathcal{O}(NTM|\mathcal{S}|^{3}|\mathcal{A}|)$ to run the algorithm across each of the $T$ epochs. 

\subsection{Real World Context: Food Rescue}
We explain the significance of our problem setup in the context of food the food rescue matching problem. 
Food rescue refers to organizations that move food donating agencies, such as restaurants or grocery stores, to food distribution agencies such as food banks. 
This movement is done through volunteers, who transport food based on trip requests from the food rescue organization. 
Examples of such organizations include 412 rescue, which matches volunteers with trips in the Pittsburgh area. 

In this scenario, arms represent volunteers, and each action $a_{i}^{t}$ determines whether to notify volunteer $i$ about trip request $t$. 
The state of a volunteer represents intrinsic information about them; the collection of states $E$ represents states where the volunteer is engaged with the food rescue system and is willing to take on requests. 
Such a state could be determined through information on the volunteer's engagement with the food rescue app, such as whether they opened the app in the past week. 
The food rescue organization could want two objectives: 1) to maintain a large pool of volunteers, which is captured by $\lambda \sum_{i=1}^{N} R_{i}(s_{i}^{(t)})$ and 2) minimizing food wastage by maximizing matches, which is captured by $\sum_{i=1}^{N} p_{i}^{(t)} a_{i}^{(t)} \mathbbm{1}[s_{i}^{(t)} \in E]$. 
For each trip, the rescue agency leverages information on current volunteers, and sends notifications, and the combination of these two determines whether volunteers take on the trip. 


==> previous_writeup/conclusion.tex <==
\section{Conclusion}

==> previous_writeup/future.tex <==
\section{Future Work}
We detail avenues for future work, detail potential opportunities, and relate these to challenges faced in other fields. 

\subsection{Unknown Transition Probabilities}
\textbf{Problem:} The computation of the Whittle index requires knowledge of the transition probabilities; however, such an assumption is largely false in reality, where transition probabilities need to be learned on the fly. 
We provide an improvement to the UCWhittle algorithm by leveraging the properties of Binomial distributions that leads to good empirical performance. 
It might be possible to prove lower bounds on this regret, combine it with our algorithm, then show that the problem is functionally solved. 

\subsubsection{UCWhittle}
The Whittle index algorithm requires perfect knowledge of the transition probabilities, $P_i$, however, some scenarios lack knowledge of these transition probabilities. 
To get around this, the \textit{UCWhittle algorithm} leverages the upper confidence bound (UCB) algorithm to estimate transition probabilities, along with confidence intervals, using sampled values~\cite{wang2023optimistic}. 
From there, the algorithm selects optimistic transitions, computing the Whittle index using each of these transitions to pick the actions. 
Formally, let $V_{i}^{(t)}(s,a,s')$ be the number of times that the transition $s \rightarrow_{a} s'$ is observed for arm $i$ until time step $t$, and let $V_{i}^{(t)}(s,a) = \sum_{s'} V_{i}^{(t)}(s,a,s^\prime)$.
Then, we can estimate the transition probability between $s$ and $s'$ with action $a$ as 
\begin{equation}
    \hat{P}_{i}^{(t)}(s,a,s') = \frac{V_{i}^{(t)}(s,a,s^\prime)}{V_{i}^{(t)}(s,a)}
\end{equation}
The confidence interval for $\hat{P}_{i}^{(t)}(s,a,s^\prime)$, $d_{i}^{(t)}(s,a,s^\prime)$ is then 
\begin{equation}
    d_{i}^{(t)}(s,a,s') = \sqrt{\frac{2|\mathcal{S}|\mathrm{log}(2|\mathcal{S}||\mathcal{A}|N\frac{t^4}{\delta})}{\mathrm{max}\{1,V_{i}^{(t)}(s,a)\}}}
\end{equation}
where $P_{i}^{(t)}(s,a,s') \in \hat{P}_{i}^{(t)}(s,a,s') \pm d_{i}^{(t)}(s,a,s')$ with probability $1-\frac{t^4}{\delta}$. 
From there, actions are picked which maximize reward optimistically, that is, the $\Bar{P}_{i} \in \hat{P}_{i}^{(t)}(s,a,s') \pm d_{i}^{(t)}(s,a,s')$, then $\bar{P}_{i}$ are selected to maximize reward. 
Such an algorithm achieves regret $\mathcal{O}(\sqrt{T \mathrm{log}(T)})$, and uses the Chernoff bound to predict the transition probability. 

\subsubsection{Improving UCWhittle}
We build on the UCWhittle algorithm by reducing the size of the confidence intervals through better bounds. 
We view the estimation of $\hat{P}_{i}^{(t)}(s,a,s')$ as the problem of estimating the parameter $\theta$ for some Bernoulli distribution given $V_{i}^(t)(s,a,s')$ successes out of $V_{i}^{(t)}(s,a)$ trials. 
Doing so allows us to leverage prior work in statistical estimation for Bernoulli distributions. 
While the normal approximation and confidence bound fails to hold for finite samples, we leverage the Wilson score interval~\cite{wilson1927probable}, which estimates $\hat{\theta}$ by solving a quadratic based on estimation of the standard deviation. 
Doing so gives us the following formula: 
\begin{equation}
    d_{i}^t(s,a,s') = \frac{z_{1-\frac{\delta}{2}}}{V_{i}^{(t)}(s,a) + z_{1-\frac{\delta}{2}}^{2}} \sqrt{\frac{V_{i}^{(t)}(s,a,s')*(V_{i}^{(t)}(s,a)-V_{i}^{(t)}(s,a,s'))}{V_{i}^{(t)}(s,a)} + \frac{z_{1-\frac{\delta}{2}}^2}{4}}
\end{equation}
We aim to prove that such a confidence interval gives provably better regret.
Doing so might solve the unknown transitions problem with Restless Multi-Armed Bandits, if we can prove lower bounds as well. 

\subsection{Multiple Types of Actions}
\textbf{Problem:} Throughout our problem statement, we assumed that exactly $K$ arms are pulled at each timestep. 
However, organizations such as food rescue platforms are not limited by the number of arms they pull. 
Instead, food rescue organizations might have multiple actions they pull, such as strong pulls, which are limited to $K$ pulls, and weak pulls, which can have as many pulls. 
This corresponds to personalized calls made by a food rescue agency for a limited number of volunteers, with notifications for the rest. 

\textbf{Solution:} Prior work has developed a PAC-learning based framework with fixed budgets for arm pulls~\cite{schumann2019making}. 
We could potentially build on this while incorporating arm transitions in the Restless bandit scenario. 
Variants of the UCB algorithm could be used, so that the arms that are the most promising (or get the best improvement) from, while the rest might be reverted to the normal notification algorithm. 

\textbf{Similar Situations:} Interviewing requests can be viewed as a situation with strong and weak pulls, where interviews are strong pulls, while phone screenings can be seen as weak pulls. 
In public health settings, there's a variety of tests that can be run to get information, with differing costs and levels of information for a PCR vs. antigen test for example. 

\subsection{Non-Linear Global Objective Functions}
\textbf{Problem:} To capture the probability of an arm responding positively to a matching request, we denoted $p_{i}^{(t)}$ to be the probability that arm $i$ is matched with request $t$ when matched. 
Using this, we aimed to maximize $\sum_{i=1}^{N} p_{i}^{(t)} a_{i}^{(t)} \mathbbm{1}[s_{i}^{(t)} \in E]$. 
However, in reality, rewards are not linear; the probability that either of two arms are matched is less than twice the probability that one arm is matched. 
In particular, our goal is to maximize 
\begin{equation}
    1-\prod_{i=1}^{N} (1-p_{i}^{(t)})^{a_{i}^{(t)}\mathbbm{1}[s_{i}^{(t)} \in E]}
\end{equation}
Solving such an equation is difficult due to its non-linearity, meaning that the Whittle index algorithm cannot be used. 
Instead, we propose several solutions to solve the non-linear matching problem leveraging variants of Q-iteration. 

\textbf{Similar Scenarios:} Our problem formulation with the generalized matching algorithm can be leveraged for any scenario where exactly $K$ arms are pulled at each iteration, and these arms are matched. 
Examples include blood donation and volunteer dispatch algorithms~\cite{van2021modeling,mcelfresh2020matching}. 
Additionally, solving this problem leads to the development of efficient algorithms that generalize the Whittle index formulation to non-linear situations. 

\subsubsection{Exact Solution: Q-Iteration}
We develop an exact algorithm to solve the matching problem using Q-learning to find optimal actions. 
The key issue with using the Whittle index algorithm with the matching objective function is the non-linearity of the global objective function, making it impossible to exactly decompose into the reward for each arm individually. 
To overcome this limitation, we perform Q-learning on all combinations of arm states; we compute $Q(\{ s_{1}^{(t)} \ldots s_{N}^{(t)} \},\{a_{1}^{(t)} \cdots a_{N}^{(t)}\})$. 
We compute this by iteratively computing 
\begin{equation}
\begin{split} 
    Q(\{ s_{1}^{(t)} \ldots s_{N}^{(t)} \},\{a_{1}^{(t)} \cdots a_{N}^{(t)}\}) = -(1-p)^{\sum_{i=1}^{N} a_{i}^{(t)} \mathbbm{1}[s_{i}^{(t)} \in E]} \\
    + \gamma \sum_{\{ s_{1}^{'(t)} \ldots s_{N}^{'(t)} \}} 
    \mathbb{P}(\{ s_{1}^{(t)} \ldots s_{N}^{(t)} \} \rightarrow \{ s_{1}^{'(t)} \ldots s_{N}^{'(t)} \} | a) V(\{ s_{1}^{'(t)} \ldots s_{N}^{'(t)} \})
    \end{split} 
\end{equation}

For matching, we can simplify the problem to whether states are in $E$ or not; doing so reduces the computational complexity of the solution, as each arm is in only one of two states.
However, despite this, the complexity of the number of state combinations is $O(2^{N})$, and because the number of actions is ${N \choose K}$, the total time complexity is $\mathcal{O}(4^{N} {N \choose K})$, far too slow for any reasonable values of $N$ and $K$. 
However, this algorithm provides an upper bound for the performance of any algorithm or approximation for the matching problem. 

\subsubsection{Heuristic: Sufficient Q Learning}
We develop a heuristic for the problem variant where $p=p_{1}^{(t)}=p_{2}^{(t)} \cdots =p_{N}^{(t)}$ for all $t$. 
We consider solutions to the full matching problem, that is, to solve 
\begin{equation}
    1-(1-p)^{\sum_{i=1}^{N} s_{i}^{t} a_{i}^{t}} + \lambda R_{i}(s_{i}^{(t)},a_{i}^{(t)})
\end{equation}
Such a problem presents a challenge because of the inability to separate our algorithm into rewards for each arm; pulling both arm 1 and 2 does not provide the sum of pulling arm 1 and pulling arm 2 independently. 
Instead, we tackle such a problem using the symmetries present in our problem, namely the symmetric dependence on each arm in the objective function. 
Traditional Whittle indices perform Q-Learning by computing $Q^{m_i}(s_{i}^{t},a_{i}^{t})$ for each state-action combination, while incorporating a subsidy. 
We instead consider \textit{sufficient Q-Learning} by leveraging sufficient statistics of the data to more accurately represent inter-arm interactions. 
We consider the statistic $T^{t}=\sum_{i=1}^{N} s_{i}^{t}$, so that we perform the following Q-iteration: 
\begin{equation}
    Q^{m_i}(s_{i}^{t},T^{t},a_{i}^{t}) = -m_i*a_{i}^{t} + \frac{1-(1-p)^{\mathrm{min}(T^{t},K)}}{T^{t}} + \lambda s_{i}^{t}
\end{equation}
In essence, the objective function takes a similar approach to Shapley values; the reward for each arm is divided up amongst the $T^{t}$ arms that could potentially be pulled for a successful match. 
We assume that for each timestep, $\mathrm{min}(T^{t},K)$ arms are pulled; more than $K$ arms cannot be pulled, and at each epoch, all arms that can result in matches (which have $s_{i}^{t}=1$) are pulled, subject to budget constraints. 
Performing Q-iteration on this objective function requires the notion of transition probabilities between values of $T$; that is, a function $p(T'|T)$. 
The value of $T'$ is impacted by two factors: the $K$ arms that are pulled, and the $N-K$ arms that are not pulled. 
We consider arms that are being pulled to have a transition probability to $s_{i}^{t}=1$ of $q_1$, and those that are not being pulled to have a transition probability of $q_0$. 
We then consider that $p(T'|T)$ is distributed according to 
\begin{equation}
    p(T'|T) \sim \mathrm{Bin}(K,q_1) + \mathrm{Bin}(N-K,q_0)
\end{equation}
where $\mathrm{Bin}(k,q_1)$ refers to the Binomial distribution with $k$ trials and probability of success $q_1$. 
We use this equation to compute transition probabilities and repeat this for each Whittle index $m_i$, resulting the computation of the minimum subsidy. 
Our algorithm results in an $\mathcal{O}(N^2)$ slowdown, resulting in a total time complexity of $\mathcal{O}(N^{3}TM|\mathcal{S}|^3|\mathcal{A}|)$, but results in more accurate Whittle index calculation through the incorporation of additional information. 

\subsubsection{Heuristic: Proximal Policy Optimization}
We consider solving the joint activity-matching problem through a neural reinforcement learning approach through the proximal policy optimization (PPO) algorithm. 
The PPO algorithm performs policy gradient to learn a policy $\pi$, which selects an action for each arm based on their states. 
This is done by jointly learning both the policy function and performing neural Q iteration by computing the advantage of each action. 

In our scenario, we aim to maximize the activity + matching problem across all agents, giving no reward if $\sum_{i=1}^{N} a_{i}^{t} > K$. 
For each epoch, we train a PPO agent to learn a policy for all states, and then use this agent across all time steps with the same collection of arms. 


\subsection{Learning Match Probabilities}
\textbf{Problem:} Solving the Whittle index requires knowledge of match probabilities, $p_{i}^{(t)}$. 
However, in reality, match probabilities are unknown, and are functions of both the arm and the request, with some inherent randomness. 
These match probabilities are also intimately related to arm preferences; if an arm has multiple pulls, then the match probability depends on the preference of that arm between each requested trip. 

\textbf{Solution:} Results from preference learning and bandit algorithms can be used to predict the values for $p_{i}^{(t)}$. 
This problem is related to contextual bandits, where the context refers to inherent information about each trip, which are then combined with information about each arm (volunteer) to determine match probabilities $p_{i}^{(t)}$. 
Solutions to this can also be combined with results from preference learning to determine what the preference is for each arm. 

\textbf{Similar Scenarios:} Unknown match probabilities can be seen in other scenarios. 
Particularly in clinical matching scenarios, such as blood donation and kidney exchange, where the match probability arises from inherent limitations in medical knowledge. 
For example, in the kidney exchange problem, determining whether a kidney can be received by a patient can only be determined through a blood test. 
Additionally, doctors may intervene on suggested matches based on clinical knowledge or cost, so that suggested cycles of patients are rejected from being matched, and are inserted back into the system. 

\subsection{Unknown Volunteer States}
\textbf{Problem:} Arm states, $s_{i}^{(t)}$, are typically unknown in practice. 
For example, understanding whether a volunteer is engaged or disengaged is hard to tell, and instead, we can only tell from observations $o_{i}^{(t)}$, which refers to observations of the state for arm $i$ at time $t$. 
Such a formulation places the problem into the partially observable Markov Decision Process (POMDP) framework. 

\textbf{Solution:} Prior work has tackled the Whittle index algorithm in the POMDP scenario~\cite{meshram2018whittle}; however, such solutions have focused on the two state situation with known randomness and a single observation. 
Later work has built on this through the use of belief states~\cite{mate2020collapsing}, however even these assume the presence of a single observation which evolves over time. 
Solving the general problem with POMDPs would provide an interesting methodological benefit, independent of any particular application, as it extends Whittle indices to a new class of processes. 

\subsection{Multiple Time Scales}
\textbf{Problem:} Throughout the paper, we assumed that a matching request occurs at every time step, $t$, and that the results of this match impacts the transition of each arm. 
However, in real-life situations, such as food rescue algorithms, the incidence of matching requests occurs more frequently than arm transitions. 
For example, volunteers might transition between states based on the results from 1 week of notifications, while food rescue trips might be batched every 20 minutes. 
Such a situation would also solve the issue where certain time iterations have no matches, as transitions occur at a larger time scale than requests. 

\textbf{Solutions:} Such a situation challenges modeling assumptions, and requires the calculation of arm transitions after multiple rewards. 
Additionally, a batching mechanism is required, so that notifications are made on some regular time interval, then notifications are made for all matching requests within that time interval. 
This delay between notifications and arm transitions might encourage different optimal policies; for example, it might be optimal to pull one arm many times before it transitions to a negative state. 

\textbf{Similar Scenarios:} Such a multi-level time scales occur in many scenarios. 
For example, in a kidney exchange scenario, requests occur on the fly, yet matches are made by batching every week or month depending on the country. 
In a public health scenario, prior work has demonstrated algorithms that occur at multiple geographic levels~\cite{bhattacharya2018restless}, so that policies are first made at a regional level, then using these predictions, individual recommendations are made. 

\subsection{Non-Markovian Transitions}
\textbf{Problem:} Transitions between states are not necesarily Markovian for arms. 
For example, a volunteer might become burned out after repeated notification requests that pile up over weeks or months. 
Most algorithms for restless bandits, including Q iteration with the Whittle index algorithm, assume Markovian transitions, as non-Markovian transitions are significantly more computationally expensive. 

\textbf{Solution:} We can estimate situations such as long-term burnout through the creation of many intermediate states which denote varying levels of burnout. 
We note that our current algorithm supports arbitrarily large numbers of states for each arm. 
Whether such an approximation leads to performance costs is unclear; it might be the situation that Markovian transitions can capture any non-Markovian situation of interest. 

\subsection{Impact of notifications without matching}
\textbf{Problem:} Not getting matched sucks. 
For arms that get notified, there's a race to get matched, with the arm which responds first getting matched. 
Volunteers, which are represented through arms, might become discouraged if they receive a notification but aren't matched. 
Additionally, the dynamics of matching itself are interesting, as it's not clear which arms might be respond first. 
It might be reliant on the preferences of the arm, where arms with more preference for a trip responding quicker. 

\textbf{Solution:} One way to solve this problem is through extra time steps, between the creation of a trip request, and the matching of volunteers. 
This new time step is where volunteers are notified, but haven't accepted yet. 
Using this formulation, different transitions can be made both after notification, and after the final match. 
Additionally, it's unclear how big such an effect is in reality, and how much it generalizes to other scenarios. 
However, there might be interesting overlap with preference learning, as the preferences impact whether arms are enthusiastic about a particular trip. 


==> previous_writeup/introduction.tex <==
\section{Introduction}
Restless multi-armed bandits (RMABs) combine the power of bandit algorithms with Markov decision processes (MDPs) to model situations where arms probabilistically transition between states, impacting the resulting reward. 
In this paradigm, $K$ out of $N$ arms are pulled each iteration, then all arms transition based on whether or not they were pulled. 
Such situations naturally occur in domains such as public health, where arms can represent different interventions, and where the success of these interventions varies based on whether or not prior interventions were taken. 
RMABs have been well studied theoretically, and the Whittle index has been shown to effectively recover optimal policies given information about arm transitions (CITATION).  
Additionally, algorithms leveraging this framework have been deployed to applications such as maternal health information (CITATION), energy-saving scheduling, and advertising.   

Prior work in RMABs has investigated the real-world feasibility of this paradigm by developing algorithms when transition probabilities are missing (CITATION). 
Other work has looked into various metrics, such as optimizing for fairness or mitigating various types of risk (CITATION). 
Much of this work relies on fast computation of the Whittle index to find optimal policies, and so prior work has improved upon this through reinforcement learning-based approaches to computing the Whittle index (CITATION). 

Much of this prior work relies on the assumption that rewards for individual arms are decoupled, which makes it difficult to extend to scenarios such as matching. 
In such scenarios, rewards are inherently based on the states of all arms; having 4 arms in a ``good'' state is not necessarily twice as good as having 2 arms in a ``good state.''
RMABs can be used to model scenarios where agents (represented by arms) can decline match requests, such as Uber drivers declining requests to pickup passengers. 
In a sense, arm pulls can represent suggestions for matching, with the goal being that as many of the $K$ arms pulled respond positively. 

In this paper, we present the joint RMAB + matching problem, and show that current Whittle-index based solutions fail to optimize for matching, even in simple scenarios. 
We develop new methods that improve both the ``activity'' of the arms pulled, and the matching success of these arms, then show that there exists a tradeoff between the two. 
We justify these methods theoretical by establishing regret bounds, showing that activity algorithms improve on prior regret bounds, while the matching algorithms achieve small regret. 
We evaluate this matching+RMAB algorithm across both synthetic data, and using real-world data from a volunteer-trip matching scenario for food donations. 

We make the following contributions: 
\begin{enumerate}
\item We combine the restless multi-armed bandit with a matching problem, and demonstrate that existing solutions to the multi-armed bandits fail to perform well for the matching problem 
\item We develop near-optimal algorithms that maximize either the activity or the matching of arms. We provably improve regret bounds for each, and show that they reach near-optimal performance
\item We explore the trade-off between activity and matching performance, and detail the trade-off curve between the two 
    
\end{enumerate}


==> previous_writeup/nonlinearity.tex <==
\section{Non-Linear Rewards}
We describe the problem of optimizing a non-linear global reward function, $R_{G}$, and propose a variety of techniques to resolve this. 

\subsection{Non-Linearity in Stationary Bandits}
We begin by describing the problem in the stationary bandit's scenario, where $T=1$, and so a single action needs to be taken. 
We consider agent $i$ to initially be in state $s_{i}^{(0)}$, then get notified to $a_{i}^{(0)}$, then based on this notification, transition to state $s_{i}^{(1)}$. 
We receive rewards from matching agents, and also from the agent's final state, resulting in maximizing 
\begin{equation}
    R_{G}(\{s_{1}^{(0)} \cdots s_{N}^{(0)}\},\{a_{1}^{(0)} \cdots a_{N}^{(0)} \}) + \sum_{i=1}^{N} R_{i}(s_{i}^{(1)})
\end{equation}
Such a problem can be computed in $\mathcal{O}({N \choose K})$, which quickly becomes infeasible for large $N$. 
We develop several algorithms in the scenario where $|\mathcal{S}| = 2$, $R_{i}(s_{i}^{(1)}) = s_{i}$, and $ R_{G}(\{s_{1}^{(0)} \cdots s_{N}^{(0)}\},\{a_{1}^{(0)} \cdots a_{N}^{(0)} \}) = 1-\prod_{i=1}^{N} (1-p_{i}s_{i}^{(0)}a_{i}^{(0)})$. 

\subsubsection{Upper Confidence Bound}
We can use an upper confidence bound-based approach to develop estimates for which arms are the best. The issue is not that we don’t know all the information, but rather the computational cost. 

We maintain a variable, $\hat{\mu_{i}}$ of the best performance when pulling arm i. We consider the $K-1$ highest values of $x$ and the $K-1$ highest values of $y$, then consider the combination of these values to get $(\bar{x},\bar{y})$. We then let $\hat{\mu_i} = \alpha F((\bar{x},\bar{y}) + (x_i,y_i)) + (1-\alpha)\max{\mu_{i,1} \cdots \mu_{i,t}}$, where $\mu_{i,t}$ is the maximum reward when pulling arm i across each iteration. At each iteration, we pull the $K$ highest arms with the largest values of $\hat{\mu_i}$; the idea is that $F((\bar{x},\bar{y})+(x_i,y_i))$ represnts a bound on the maximum performance, while $\max \mu_{i,1} \cdots \mu_{i,t}$ is the actual best performance we get. We then let $\alpha = \frac{1}{\sqrt{n}}$ so that the actual performance becomes more important with the largest $N$.

\subsubsection{Dynamic Programming}
We consider a dynamic programming based solution based on the following recurrence

$\mathrm{DP}[k][n][e] = \max(\mathrm{DP}[k][n-1][e],\mathrm{DP}[k-1][n-1][\frac{e x_n}{\epsilon}] + y_n \mathrm{ if s_i=1},\mathrm{DP}[k-1][n-1][e] + y_n \mathrm{ if s_i=0})$, where $\epsilon$ is some small number so we can deal with floating points, such as 0.01. The base case is $\mathrm{DP}[0][n][e] = \mathrm{DP}[k][0][e] = 1-e$. This program has space and time complexity $\mathcal{O}(\frac{NK}{\epsilon})$. 

The key idea is that we store three values at each iteration: K, the number of spots still left, N, which represents the values we’re considering, and e, the probability that we don’t match so far. We represent e as an integer, by storing $\frac{e}{\epsilon}$, which is where the approximation comes from in this algorithm.

\subsection{Reward Decomposition}

\subsection{Monte-Carlo Tree Search}

\subsection{Deep Reinforcement Learning}

\subsection{Dynamic Programming}

==> previous_writeup/related.tex <==
\section{Related Works}
\paragraph{Multi-Armed Bandits} Work in Restless Multi-Armed Bandits, which adds MDPs to bandit arms, has looked into applications in public health settings, along with minmaxing regret and including notions of fairness. 

\paragraph{Matching} Working in matching has leveraged a variety of reinforcement learning concepts, including Deep Q networks to learn the value for a particular match. 

\paragraph{Notification} Notification algorithms, such as those for blood donations and food rescue, leverage matching and bandits to deal with the online uncertainty inherent in the problem. 

==> previous_writeup/results.tex <==
\section{Experiments}
\subsection{Datasets}
TODO: Detail the synthetic + food rescue datasets

\subsection{Metrics}
TODO: Detail our computation of activity, matching metrics

\subsection{Heuristics}
In addition to our Whittle-based solution to the matching problem, we consider three heuristics for matching: 
\begin{enumerate}
    \item \textbf{Zero Step Myopic} - We let $a_{i}^{(t)} = 1$ if $s_{i}^{(t)} = 1$, breaking ties arbitrarily. If $\sum_{i=1}^{N} a_{i}^{(t)} < K$, we select the remaining arms to pull using the one step myopic detailed below
    \item \textbf{One Step Myopic} - We let $a_{i}^{(t)} = 1$ for the arms which maximize $s_{i}^{(t)} * P_{i} (s_{i}^{(t)},1,1)$, essentially aiming to maximize the number of arms in an acceptable state for matching. 
    \item \textbf{Infinite Step Myopic} - We consider an extension of one step myopic, where instead we consider the arms that maximize the probability after $B \rightarrow \infty$ steps. That is, we consider the steady state probability for arm $i$ being in state $1$ (which represents the set $E$) after pulling the arm for $B$ iterations. We compute this through a steady state vector by solving the eigenvectors for $P_i(s,1,s')$, and computing the long-run probability of being in state 1
\end{enumerate}


\subsection{Comparison of Activity-Only Algorithm}
TODO: Create an optimal activity algorithm + compare it on synthetic data + food rescue data

\begin{table}
    \centering
    \begin{tabular}{@{}lccc@{}}
        \toprule
        Algorithm & \multicolumn{1}{c}{Bandit Perf.} & \multicolumn{1}{c}{Matching Perf.} \\ 
        \midrule
        Random & $3.06 \pm 0.01$ & $0.984 \pm 0.001$ \\ 
        Optimal & $3.55 \pm 0.04$ & $0.996 \pm 0.001$ \\ 
        WIQL & $2.98 \pm 0.04$ & $0.978 \pm 0.004$ \\ 
        Extreme & $2.92 \pm 0.02$ & $0.987 \pm 0.002$ \\ 
        UCB & $2.90 \pm 0.01$ & $0.975 \pm 0.005$ \\ 
        Fixed & $3.14 \pm 0.04$ & $0.983 \pm 0.002$ \\ 
        QP & $2.94 \pm 0.03$ & $0.987 \pm 0.000$ \\ 
        Value & $2.93 \pm 0.02$ & $0.986 \pm 0.001$ \\ 

        \bottomrule
    \end{tabular}
    \caption{Bandit and Matching Performance}
\end{table}

\begin{figure}
    \centering 
    \includegraphics[width=200pt]{figures/normal_improvement.pdf}
    \caption{Fixing the bug + using normal distribution improves activity}
\end{figure}

\subsection{Performance of Matching Algorithm}
TODO: Create an optimal empirical matching algorithm + compare it with the best possible if transitions were known

\subsection{Pareto efficiency}
TODO: Find the best possible pareto algorithm, and see what the tradeoff is



==> previous_writeup/rmab.tex <==
\section{Prior work: Restless Multi-Armed Bandits (RMABs)}
\label{sec:rmab}
We introduce restless multi-armed bandits and describe prior work in finding optimal actions in this paradigm.  
We detail two existing algorithms: the Whittle index, a provably optimal algorithm for determining arm pulls in the RMAB problem, and the UCWhittle algorithm, which approximates the Whittle index algorithm when transition probabilities are unknown. 

\subsection{Defining Restless Multi-Armed Bandits}
We formally introduce restless multi-armed bandits (RMABs), which extend multi-armed bandits (MABs) with state-evolving arms. 
Each arm of an RMAB can be thought of as a Markov Decision Process (MDP), and the pulling or abstaining of an arm performs an action. 
Formally, we consider an MDP $(\mathcal{S},\mathcal{A},R,\mathcal{P}_i)$, where $\mathcal{S}$ the set of states, shared between arms, $\mathcal{A}$ is the action space, which is either pulling or not pulling the arm, $R: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$ is the reward function, and $\mathcal{P}_i: \mathcal{S} \times \mathcal{A} \times \mathcal{S} \rightarrow \mathbb{R}$ is a transition matrix, unique to each arm. 

Let the state of arm $i$ at time $t$ be $s_{i}^{(t)} \in \mathcal{S}$, and let the action taken for arm $i$ at time $t$ be $a_{i}^{(t)} \in \{0,1 \} = \mathcal{A}$. 
Actions, $a_{i}^{(t)}$ are determined using information about the state, $s_{i}^{(t)}$, and after playing the action, the state of arm $i$ changes to $s_{i}^{t+1}$, which is distributed proportional to $P_i(s_{i}^{(t)},a_{i}^{(t)},s')$, where $\sum_{s^\prime} P_i(s_{i}^{(t)},a_{i}^{(t)},s^\prime) = 1$. 
We let $\mathbf{s}$ be the vector, $\mathbf{s} = [s_{1}^{t} \cdots s_{N}^{t}]$, and similarly, we let $\mathbf{a}$ be the equivalent vector for actions, $\mathbf{a} = [a_{i}^{t} \cdots a_{N}^{t}]$.  
Additionally, let $\mathcal{P} = [P_{1} \cdots P_{N}]$. 
At each time step, we may only pull at most $K$ of the arms, so $\sum_{i=1}^{N} a_{i}^{(t)} \leq K$, for all $t$. 
Our aim to select actions according to a policy $\pi: \mathcal{S}^{N} \rightarrow \mathcal{A}^{N}$ that maximize rewards across all arms, discounted by a factor $\gamma$. 
In total, we aim to solve the following optimization problem

\begin{equation}
\begin{array}{ll@{}ll}
\max_{\pi}  \mathbb{E} _{(\mathbf{s},\mathbf{a})\sim (\mathcal{P},\pi)}& \displaystyle  \sum_{t=0}^{\infty} \gamma^{t} \sum_{i=1}^{N} R(s_{i}^{(t)},a_{i}^{(t)}) & &\\
\text{subject to}&                                                & a_{i}^{(t)} \in [0,1]           &i=1 ,\dots, n\\
                 &\displaystyle\sum\limits_{i=1}^{N}              & a_{i}^{(t)} \leq K \forall t   & \\
\end{array}
\end{equation}


\subsection{Whittle Index Policies}
\label{sec:whittle}
Despite the PSPACE complexity for finding optimal algorithms for RMABs~\cite{papadimitriou1994complexity}, the Whittle index algorithm leverages the structure of RMABs to develop provably optimal solutions for a subset of ``indexable'' bandits~\cite{whittle1988restless}. 
The Whittle index algorithm associates each arm with a ``whittle index'', $w_i$, then selects the $K$ arms with the highest values for $w_i$. 
The index represents the amount of penalty necessary to encourage arm $i$ not to be pulled, and captures the benefit of pulling arm $i$, with higher values of $w_i$ indicating more benefit from pulling arm $i$. 
To compute $w_i$, we consider the Q value for arm $i$ with a subsidy $m_i$ as $Q_{i}^{m_i}(s_i,a_i) = -m_i*a_i + R_{i}(s_i,a_i) + \gamma \sum_{s_i' \in \mathcal{S}} P_{i}(s_i,a_i,s_i') V_{i}^{m_i}(s_i')$, where $V_{i}^{m_i}(s_i) = \mathrm{max}_{a} Q_{i}^{m_i}(s_i,a)$. 
When $Q_{i}^{m_i}(s_i,1) > Q_{i}^{m_i}(s_i,0)$, we know that the subsidy was not high enough, so it's still beneficial to pull arm $i$, while if $Q_{i}^{m_i}(s_i,1) < Q_{i}^{m_i}(s_i,0)$, the subsidy is too high, so pulling the arm is overly penalized. 
Therefore, to compute the Whittle index, we consider the smallest subsidy so that $Q_{i}^{m_i}(s_i,1) \leq Q_{i}^{m_i}(s_i,0)$; that is 
\begin{equation}
    w_i = \text{min}_{m_i} \{m_i: Q_{i}^{m_i}(s_i,1) \leq Q_{i}^{m_i}(s_i,0)\}
\end{equation}
Such a value can be quickly computed through a binary search on $m_i$, with each iteration of a binary search requiring solving for Q values for each arm. 
Whittle indices allow for solutions to be decomposed into the solutions for individual arms so that each arm can be solved independently, which can then be used to compute indices. 






==> previous_writeup/theory.tex <==
\section{Theoretical Analysis}
\subsection{Regret bounds of activity Algorithm}
TODO: We prove that our strategy improves the regret bounds for the activity of the notification algorithm over the current state of the art. 

\subsection{Indexability of Whittle + Matching}
TODO: Why can we use the Whittle algorithm; is it indexable? 

\subsection{Regret bounds of UC Whittle for Matching}
TODO: How well does our matching algorithm do when the transition probabilities aren't known


==> sections/checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We present algorithms for \abr{rmab-g}s, prove approximation bounds, and verify empirical performance. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In Section~\ref{sec:conclusion}, listed out limitations. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Proofs for all Theorems can be found in Appendix~\ref{sec:proofs_difficulty} and Appendix~\ref{sec:proofs_index}. All Theorems have assumptions, etc. listed out. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: List out experimental details in Appendix~\ref{sec:experimental_details}, Appendix~\ref{sec:policy_details}, and Appendix~\ref{sec:baseline_details}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We plan to provide the code in the supplemental materials. We plan to release our synthetic dataset; our food rescue dataset is proprietary, so we are unable to release this. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Detail optimizers, etc. for the \abr{dqn} baseline in Appendix~\ref{sec:baseline_details}. General experimental details are in Appendix~\ref{sec:experimental_details}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Plot the standard error for plots to show statistical significance
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In Appendix~\ref{sec:experimental_details}, detail the resources used
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We conform to the code of ethics
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have a broader impacts sections which discusses the societal impacts
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No pretrained models, etc.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Code packages that are used are referenced, and any datasets are referenced
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No new assets from this paper
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No human subjects
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No human studies
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


